"What makes a question inquisitive?" A Study on Type-Controlled Inquisitive Question Generation

We propose a type-controlled framework for inquisitive question generation. We annotate an inquisitive question dataset with question types, train question type classifiers, and finetune models for type-controlled question generation. Empirical results demonstrate that we can generate a variety of questions that adhere to specific types while drawing from the source texts. We also investigate strategies for selecting a single question from a generated set, considering both an informative vs.~inquisitive question classifier and a pairwise ranker trained from a small set of expert annotations. Question selection using the pairwise ranker yields strong results in automatic and manual evaluation. Our human evaluation assesses multiple aspects of the generated questions, finding that the ranker chooses questions with the best syntax (4.59), semantics (4.37), and inquisitiveness (3.92) on a scale of 1-5, even rivaling the performance of human-written questions.

==> content/intro_orig.tex <==
\section{Introduction} \label{section:intro}

\Kevin{I created latex commands for model names and the inquisitive dataset so that we can get uniformity in the text and more easily make changes in the future. I think the current naming scheme can be improved, but it's a starting point (and it will be much easier to experiment with changing it once we are using the appropriate latex commands whenever we want to mention them)}

Recently, there has been a growing interest in the task of automatic question generation (AQG) from text \cite{du-etal-2017-learning, sun-etal-2018-answer, kumar2020clarq}.  AQG is useful in building conversational AI systems \cite{bordes2016learning, gao-etal-2019-interconnected}, generating synthetic examples for question answering systems \cite{alberti-etal-2019-synthetic, 10.5555/3454287.3455457, sultan-etal-2020-importance}, and 
%most importantly - 
educational applications, such as assessment of reading comprehension, intelligent tutoring, instructional games, to name a few \cite{ICWSM18LearningQ, flor-riordan-2018-semantic}. In the majority of such research, AQG focuses on generating factual questions\----questions that tend to ask about specific information that appears in the text (i.e., ``who did what to whom'') \cite{du-etal-2017-learning, flor-riordan-2018-semantic}.  Models are often trained on factual question answering datasets such as SQuAD \cite{rajpurkar-etal-2016-squad}. 

%Given a source text and optional information (e.g., a larger context, gold answers, etc.) this challenging task comprises of automatically asking questions based on the source text (or, asking question about a specific span of text from the source text \cite{ko2020inquisitive}).



   

%As pointed out by \cite{nema2019let},
\iffalse 
Automatic question generation (AQG) is first introduced for reducing cost on educational purposes. However, this leads to the current circumstances where the majority work is aimed to generate questions based on informative factorial datasets, such as Wikipedia. 
\Debanjan{Start with a more generic introduction.  what is AQG - recent related work and its applications, such as education. Then bring the motivation - majority of the work is based on informative factual dataset such as wiki and not deeper inquisitive. }
\fi 

\begin{table}[t]
\centering
\setlength{\tabcolsep}{15pt}
    \scalebox{0.72}{

\begin{tabular}{ |p{9cm}| }
\hline
\\
Source sentence: The bank holding company also reported that third-quarter profit dropped 41\%, to \$42.7 million, or 61 cents a share, from the year-earlier \$72.3 million, or \$1.04 a share.\\
        \\[6pt]
        Informative questions:\\
        1. How much did the profit drop? \\
        2. How much the third quarter profit?
        \\[6pt]
        Inquisitive questions:\\
        1. How did the third-quarter profit drop?\\
        2. What caused the drop in profit? \\
\\
\hline


\end{tabular}
}
\caption{Examples of informative and inquisitive questions.} 
\label{table:example}
\end{table}

%This might include asking about background information, elaborate some under-specified facts, and causal reasoning behind some particular actions described in the text.

Instead of asking factual questions with answers already present in the text, \newcite{ko2020inquisitive} argue that human readers instinctively ask  %inquisitive
questions that are curiosity-driven, answer-agnostic, and seek a high-level understanding of the document being read. They refer to such questions as \emph{inquisitive questions}. Inquisitive questions pursue deeper information than typical factual questions \citep{clark2020tydi}. Consider the example in  Table~\ref{table:example}. The source sentence and the inquisitive questions are from the dataset described in \newcite{ko2020inquisitive} (henceforth \inquisitive\Kevinin{I created a command for this and set it to match the formatting used by Ko et al}; for details, see Section \ref{section:data}). For comparison, the informative questions are generated by training a transformer model (BART \cite{lewis-etal-2020-bart} with default parameters) on SQuAD \cite{rajpurkar-etal-2016-squad}, which is a popular dataset for AQG research. The informative questions seek surface-level information (e.g., ``how much did the profit drop?'') whereas the inquisitive questions are seeking deeper information (e.g., ``what caused the drop in profit?''), namely the reason for the profit drop.     


%This circumstance would lead to differences between the inquisitive questions which are seeking deeper information and factoid questions that could be easily answered from the context \citep{clark2020tydi}. An example is listed in Figure~\ref{inquisitive} to show the differences between informative and inquisitive questions. We could find the answer (41\%) to the informative question in the source sentence.


%However, we need more information to answer the inquisitive questions, namely the method/reason for the profit drop.
%\Debanjan{explain the figure - example by example}

%Instead of generating factoid questions that have answers on the surface of text, more and more works start to focus on asking inquisitive questions that are more creative, with a style of curious dialogues or interactions \citep{10.1162/tacl_a_00276, scialom-staiano-2020-ask, ko2020inquisitive}. However, they are either limited by the nature of datasets, or focus less on improve performance of pretrained models.



\iffalse


\begin{center}{t}
\small
\fbox{%
    \parbox{0.8\linewidth}{%
        Source sentence: The bank holding company also reported that third-quarter profit dropped 41\%, to \$42.7 million, or 61 cents a share, from the year-earlier \$72.3 million, or \$1.04 a share.
        \\[6pt]
        Informative question:\\
        How much did the profit drop?
        \\[6pt]
        Inquisitive questions:\\
        1. How did the third-quarter profit drop?\\
        2. What caused the drop in profit?
    }
}
\end{center}
\begin{minipage}{\linewidth}
\captionof{figure}{Examples of auto-generated informative question and inquisitive questions, which are generated by models trained on SQuAD \citep{rajpurkar-etal-2016-squad} and INQUISITIVE \citep{ko2020inquisitive} respectively. \label{inquisitive}}
\end{minipage}

\fi

Based on the \inquisitive dataset, in this work, we generate inquisitive questions that are grounded upon theoretical underpinnings regarding specific rhetorical question types (see Section \ref{subsection:qannot}). \Kevinin{The previous sentence has a lot happening in it. I think we should first introduce the idea of training models to generate inquisitive questions from \inquisitive, then say how this method is insufficient for inquisitive questions due to the presence of multiple natural question type categories in the data, etc etc}
To this end, we first annotated 1500 questions from the training partition of the \inquisitive dataset to identify the question types, such as questions that inquire about background information, ask about the cause of an event, ask to elaborate under-specified facts, etc. We finetune a RoBERTa model \cite{liu2019roberta} to classify the question types on the rest of the dataset. Finally, the question types are used as control codes \cite{keskar2019ctrl,krause-etal-2021-gedi-generative} with BART \cite{lewis-etal-2020-bart}, a large pretrained transformer model, to generate inquisitive questions. Such probing inquisitive questions come naturally to humans and are useful in knowledge acquisition and building reasoning skills for students \cite{ko2020inquisitive, cao-wang-2021-controllable}. \Kevinin{The previous sentence does not seem to flow from what came before it. It feels more like high-level motivation for inquisitive questions in general. I think it was used to motivate ranking, but I think the motivation for ranking is just that in some cases we want a single question or a ranked list of questions, and for that purpose we need ways to automatically choose a question or rank questions. That is, the value of ranking is not limited to educational contexts.} Given, the models are trained to generate a variety of questions based on a specific source text (we are using six question types as control codes) we investigate two  scenarios to select the \emph{best} questions. In the first scenario, the model(s) generate all six types of questions and then we select the \emph{best} question predicted by an inquisitive vs. informative question classifier (denoted below as \cssnqt). 
%as \emph{context-source-span-nqtype} or for brevity, \cssnqt in section \ref{section:method} and section \ref{section:result}, respectively).
Here, gold questions from the SQuAD dataset are used as the informative questions. In the second scenario, expert annotators first rank the questions from a subset of generated questions and then we train a pairwise ranker on that subset to select the best questions (denoted as \cssrankqt).  %\emph{context-source-span-rank} or, \emph{cssrankqt} in section \ref{section:method} and section \ref{section:result}). 
We conduct an automatic evaluation that measures the extent of repeating source text and gold questions into generated questions and observe that question generated from \cssrankqt %\emph{context-source-span-rank} model 
are the most novel questions and used the article text most (section \ref{subsection:humeval}). \Kevinin{I'm a little confused by the claims in the previous sentence.. \cssrankqt does have the highest numbers in the Article columns in Table 5...}
Likewise, we report a large-scale human evaluation via Amazon Mechanical Turk  and demonstrate that questions generated from the same model have the best syntax (4.78) and inquisitiveness (4.16) on a scale of 1-5 
%(1 is the lowest and 5 is the highest, 
(Section \ref{subsection:humeval}). Our annotations and code will be made available. \Kevinin{Can we also release the MTurk judgments?}
%The \inquisitive corpus with the annotated question types and code will be released.   
\Kevinin{I think this intro is a good start. As we discussed in our meeting, it would be good to spend a little less space on motivating inquisitive questions (as that has already been done by Ko et al) and focus more on motivating what we did and what our contributions are. E.g., motivate question types, describe what we did regarding them, then say why it's useful (one can generate one or multiple questions of specific question types for any span; e.g., an educator can see suggested questions for a specific span when designing quizzes or choosing essay questions). However, there are cases where one may want a single high-quality question for a span. For that case, we develop and experiment with methods for ranking inquisitive questions, etc etc}



\Debanjan{need to add the usefulness.}\Kevinin{agreed}
%questions with BART \citep{lewis-etal-2020-bart} on INQUISITIVE dataset \citep{ko2020inquisitive}. It is a transformer-based model that could be seen as generalizing both GPT and BERT schemes with a bidirectional encoder and an autoregressive decoder. BART is particularly fit for generation tasks with its decoder structure.\Debanjan{explain what is BART and why you are using this.}

%Focused on the nature of the questions, we annotate 1550 questions that sampled from the training set to 7 question types, and then build a classifier with RoBERTa\citep{liu2019roberta} to label the remaining data. Since controllable text generation with semantic perturbations is widely used for style transfer or generation enhancement, we use the question types as control codes to generate questions, and evaluate our predictions with both automatic metrics and human evaluations.
%\Debanjan{write the above as ``motivations'' - what motivate you to use conditional generations and discriminative models - please see the story paper introduction here}
%\Debanjan{write the above/below as contributions.}

==> content/related_lg.tex <==
\section{Related Work}
% While many works have been done on generating factoid questions \citep{rajpurkar-etal-2016-squad, 10.1162/tacl_a_00276} as these kind of questions are often applied for language learning, inquisitive question generation is a harder task with its answer-agnostic, curiosity-driven intrinsics. Without the limitations of answers, it's crucial to control our generations.
While inquisitive question generation is more difficult and diverse with its answer-agnostic, curiosity-driven intrinsics \citep{}, it's crucial to control the generation for better questions.

Multiple attributes could be selected to control text generation recently, e.g. emotions \citep{liu-etal-2021-dexperts}, styles \citep{} and topics \citep{}. Some works modified the training process \citep{DBLP:journals/corr/abs-2107-07150}, and some works control in the decoding process \citep{liu-etal-2021-dexperts}. 
% For the former approach, semantic control with control codes. PP

According to \newcite{article_review}, questions generated from ontologies are more varied than those generated from text. We could treat the question types with conventional question generation methods, i.e. template-based, syntactic-based and semantic-based. The template-based approach is to use wh-words as question types (e.g. What, Who, How), which could also be used as leading words of questions and fused into question generation \citep{agarwal-etal-2011-automatic, zhou-etal-2019-question, wu-etal-2020-question}. The syntactic-based approach applies parser for classifying types \citep{mazidi-tarau-2016-infusing}. And the semantic approach is varied according to tasks and datasets. \newcite{Chen2009GeneratingQA} specifies three kind of questions about `conditional context', `temporal information' and `possibility and necessity' on topic. \newcite{cao-wang-2021-controllable} modified their question types from \citep{DBLP:journals/dad/OlneyGP12}, and their questions types are ranked by levels of cognition, and take answerers' opinions into consideration (e.g. judgemental) as they use answers as model input instead of context sentences.
% \citep{DBLP:conf/acl/HeLLLZXLWWSLWW18}

\Lingyu{In fact, Cao and Wang's qustion types are pretty similar to ours, only with different names. Their question types are more with 10 categories. }

In this paper, we applied semantic question types as control codes to generate questions for inquisitive dataset. 

% \citep{nema-khapra-2018-towards} proposes that answerablility has poor correlation with BLEU scores. \citep{sultan-etal-2020-importance} says standard QG evaluation metrics such as BLEU, ROUGE and METEOR are inversely correlated with diversity.
